Little Red Dots and their Progenitors from Direct Collapse Black Holes

The James Webb Space Telescope (JWST) has discovered a new population of objects, the Little Red Dots (LRDs), characterized by V-shaped spectra indicative of strong breaks around the Balmer limit and compact morphology that gave them their name. A popular explanation is that they are a sub-population of active galactic nuclei/supermassive black holes (AGN/SMBHs) predominantly found in the high-redshift Universe ($z\gtrsim3$). Similarly, direct collapse black holes (DCBHs), theorized to form from collapsing massive, extremely metal-poor gas clouds, have been invoked to explain high-redshift quasars, the most massive AGN sub-population. Here, we employ the semi-analytical code A-SLOTH to produce a population of DCBHs and compare them against observed LRD demographics and properties. Specifically, we compare the DCBH-seeded SMBH population against the standard stellar-remnant seeds and find that DCBH models agree better with observed LRD population statistics and host halo properties. Furthermore, for the most extreme and earliest LRD detections, interpreted to be systems with an AGN but little stellar component, DCBHs are able to reproduce the observed spectral shape and properties under multiple scenarios - high dust attenuation or AGN surrounded by dense gas - that have been proposed to explain the unique shape of LRD spectra. Even when super-Eddington accretion, invoked previously to explain the nature of LRDs, is enforced on stellar remnant seeds, the spectral characteristics of extreme LRDs cannot be reproduced. We emphasize the importance of gas-metallicity observations as an additional dimension besides the widely used SMBH-stellar mass ratios to further constrain the progenitors of LRDs.

==> abbrev.tex <==
% the list from ApJ
\newcommand{\aj}{AJ}
\newcommand{\apj}{ApJ}
\newcommand{\apjl}{ApJ}
\newcommand{\apjlett}{ApJ}
\newcommand{\apjs}{ApJS}
\newcommand{\apjsupp}{ApJS}
\newcommand{\aap}{A\&A}
\newcommand{\astap}{A\&A}
\newcommand{\araa}{ARA\&A}
\newcommand{\aapr}{A\&A Rev.}
\newcommand{\aaps}{A\&AS}
\newcommand{\mnras}{MNRAS}
\newcommand{\pasp}{PASP}
\newcommand{\apss}{Ap\&SS}
\newcommand{\pasj}{PASJ}
\newcommand{\nat}{Nature}
\newcommand{\sci}{Science}
\newcommand{\skytel}{S\&T}
\newcommand{\memras}{MmRAS}
\newcommand{\qjras}{QJRAS}
\newcommand{\jrasc}{JRASC}
\newcommand{\baas}{BAAS}
\newcommand{\iauc}{IAU Circ.}
\newcommand{\iaucirc}{IAU Circ.}
\newcommand{\aplett}{Astrophys. Lett.}
\newcommand{\apspr}{Astrophys. Space Phys. Res.}
\newcommand{\bain}{Bull. Astron. Inst. Netherlands}
\newcommand{\fcp}{Fund. Cosmic Phys.}
\newcommand{\aipconf}{AIP Conf. Proc.}
\newcommand{\aspconf}{ASP Conf. Ser.}
\newcommand{\asslconf}{Ap\&SSL Conf. Ser.}
\newcommand{\procspie}{Proc. SPIE}
\newcommand{\maps}{MAPS}
\newcommand{\planss}{Planet. Space Sci.}
\newcommand{\ssr}{Space Sci. Rev.}
\newcommand{\ao}{Appl. Opt.}
\newcommand{\applopt}{Appl. Opt.}
\newcommand{\solphys}{Sol. Phys.}
\newcommand{\pra}{Phys. Rev. A}
\newcommand{\prb}{Phys. Rev. B}
\newcommand{\prc}{Phys. Rev. C}
\newcommand{\prd}{Phys. Rev. D}
\newcommand{\pre}{Phys. Rev. E}
\newcommand{\prl}{Phys. Rev. Lett.}
\newcommand{\rmp}{Rev. Mod. Phys.}
\newcommand{\jcap}{J. Cosmology Astropart. Phys.}
% my additions

